MuSHRoom: Multi-Sensor Hybrid Room Dataset for Joint 3D Reconstruction and Novel View Synthesis

Metaverse technologies demand accurate, real-time, and immersive modeling on consumer-grade hardware for both non-human perception (e.g., drone/robot/autonomous car navigation) and immersive technologies like AR/VR, requiring both structural accuracy and photorealism. However, there exists a knowledge gap in how to apply geometric reconstruction and photorealism modeling (novel view synthesis) in a unified framework. To address this gap and promote the development of robust and immersive modeling and rendering with consumer-grade devices, we propose a real-world Multi-Sensor Hybrid Room Dataset (MuSHRoom). Our dataset presents exciting challenges and requires state-of-the-art methods to be cost-effective, robust to noisy data and devices, and can jointly learn 3D reconstruction and novel view synthesis instead of treating them as separate tasks, making them ideal for real-world applications. We benchmark several famous pipelines on our dataset for joint 3D mesh reconstruction and novel view synthesis. Our dataset and benchmark show great potential in promoting the improvements for fusing 3D reconstruction and high-quality rendering in a robust and computationally efficient end-to-end fashion. The dataset and code are available at the project website: https://xuqianren.github.io/publications/MuSHRoom/.

==> WACVAuthorKit/sec/exp/ablation.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h]

\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccc}
\toprule
\multirow{3}{*}{Method}            & \multicolumn{5}{c}{\multirow{2}{*}{Reconstruction quality}} & \multicolumn{6}{c}{Rendering quality}                                \\ \cline{7-12}
                                   & \multicolumn{5}{c}{}                                        & \multicolumn{3}{c}{Test within a single sequence} & \multicolumn{3}{c}{Test with a different sequence} \\ \cline{2-12}
                                   & \textbf{Acc} $\downarrow$ & \textbf{Comp} $\downarrow$ & \textbf{C-}$\ell_1$ $\downarrow$ & \textbf{NC} $\uparrow$& \textbf{F-score} $\uparrow$& \textbf{PSNR} $\uparrow$& \textbf{SSIM}  $\uparrow$& \textbf{LPIPS} $\downarrow$& \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$   \\ \midrule
Volumetric Fusion (original depth) & 0.0178    & 0.0218     & 0.0198   & 0.8514    & 0.9217   & 14.61      & 0.6920     & 0.3774    &  12.90        &   0.6634       &  0.4150        \\
Volumetric Fusion (inpainting depth) & 0.0207    & 0.0212     & 0.0210    & 0.8407    & 0.9143    & 14.92      & 0.6873     & 0.3950    &  13.84        &   0.6556       &   0.4170       \\
NeuS-facto (original depth)        & 0.0145    &  0.0183   & 0.0164    & 0.9121    & 0.9565   & 21.08     & 0.7658     & 0.2198    &   \textbf{22.37}       &   \textbf{0.8483}       &   \textbf{0.1396}       \\
NeuS-facto (inpainting depth)      & \textbf{0.0136}     &  \textbf{0.0161}    & \textbf{0.0149}    & \textbf{0.9130}   & \textbf{0.9655}    & \textbf{21.21}      & \textbf{0.7709}     & \textbf{0.2132}    &   21.98       &  0.8465        &  0.1427        \\ \bottomrule

\end{tabular}%
}
\caption{The ablation study of inpainting depth and two-head structure. Test within a single sequence means we uniform sample test frames from a single sequence and train on all left frames. Test with a  different sequence means we train on one sequence and test on another individual sequence.}
\label{exp:ablation}

\end{table*}

==> WACVAuthorKit/sec/exp/ablation_structure.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{Device} & \multirow{2}{*}{Room}     & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Test within a\\ single sequence\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Test with a\\ different sequence\end{tabular}} \\ \cline{4-9} 
                        &                           &                          & \textbf{PSNR} $\uparrow$                       & \textbf{SSIM}  $\uparrow$                         & \textbf{LPIPS} $\downarrow$                        & \textbf{PSNR} $\uparrow$                         & \textbf{SSIM}  $\uparrow$                          & \textbf{LPIPS} $\downarrow$                          \\ \hline
\multirow{6}{*}{Kinect} & \multirow{3}{*}{activity} & NeuS-facto               & 19.53                       & 0.7258                       & 0.3356                       & 20.18                        & 0.7707                        & 0.2750                        \\
                        &                           & w/o DA                   & 20.30                       & 0.7379                       & 0.3222                       & 21.06                        & 0.7864                        & \textbf{0.2531}               \\
                        &                           & Ours                     & \textbf{20.89}              & \textbf{0.7509}              & \textbf{0.3221}              & \textbf{21.33}               & \textbf{0.7919}               & 0.2534                        \\
                        & \multirow{3}{*}{honka}    & NeuS-facto               & 19.40                       & 0.7759                       & 0.2658                       & 22.45                        & 0.8505                        & 0.1616                        \\
                        &                           & w/o DA                   & 20.70                       & 0.7962                       & \textbf{0.2440}              & \textbf{24.04}               & 0.8671                        & \textbf{0.1401}               \\
                        &                           & Ours                     & \textbf{20.86}              & \textbf{0.8000}              & 0.2584                       & 23.59                        & \textbf{0.8683}               & 0.1527                        \\ \hline
\multirow{6}{*}{iPhone} & \multirow{3}{*}{computer} & NeuS-facto               & 16.59                       & 0.6636                       & 0.4197                       & 15.83                        & 0.6327                        & 0.4321                        \\
                        &                           & w/o DA                   & 19.45                       & 0.7248                       & 0.3661                       & 17.66                        & 0.6769                        & 0.3835                        \\
                        &                           & Ours                     & \textbf{20.10}              & \textbf{0.7411}              & \textbf{0.3530}              & \textbf{18.10}               & \textbf{0.6894}               & \textbf{0.3649}               \\
                        & \multirow{3}{*}{sauna}    & NeuS-facto               & 17.37                       & 0.6791                       & 0.5354                       & 16.78                        & 0.6585                        & 0.5330                        \\
                        &                           & w/o DA                   & 19.31                       & \textbf{0.7043}              & 0.4716                       & \textbf{18.20}               & 0.6742                        & \textbf{0.4760}               \\
                        &                           & Ours                     & \textbf{19.82}              & 0.7126                       & \textbf{0.4700}              & 18.61                        & \textbf{0.6805}               & 0.4778                        \\ \hline
\end{tabular}%
}
\caption{The ablation study of two-head structure and data augmentation (DA) in rendering quality. Two-head structure can improve the overall performance. DA is much more effective for larger rooms. }
\vspace{-0.5cm}
\end{table}

==> WACVAuthorKit/sec/exp/comparison.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table.xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table.xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccc}
\hline
                                                                           &                          &                           & \multicolumn{5}{c}{}                                                                                                                                                                                                                                                                  & \multicolumn{6}{c}{Rendering quality}                                                                                                                                                                                                                                                                                                       \\ \cline{9-14} 
                                                                           &                          &                           & \multicolumn{5}{c}{\multirow{-2}{*}{Reconstruction quality}}                                                                                                                                                                                                                          & \multicolumn{3}{c}{Test within a single sequence}                                                                                                                    & \multicolumn{3}{c}{Test with a different sequence}                                                                                                                   \\ \cline{4-14} 
\multirow{-3}{*}{Room}                                                     & \multirow{-3}{*}{Device} & \multirow{-3}{*}{Methods} &  \textbf{Acc} $\downarrow$                           & \textbf{Comp} $\downarrow$                          & \textbf{C-}$\ell_1$ $\downarrow$                          & \textbf{NC} $\uparrow$                            & \textbf{F-score} $\uparrow$                       & \textbf{PSNR} $\uparrow$                         & \textbf{SSIM} $\uparrow$                          & \textbf{LPIPS} $\downarrow$                         & \textbf{PSNR} $\uparrow$                         & \textbf{SSIM} $\uparrow$                          & \textbf{LPIPS} $\downarrow$                        \\ \hline
                                                                           &                          & Volumetric Fusion         & {\color[HTML]{000000} 0.0207}                         & {\color[HTML]{000000} 0.0212}                         & {\color[HTML]{000000} 0.0210}                         & {\color[HTML]{000000} 0.8407}                         & {\color[HTML]{000000} 0.9143}                         & {\color[HTML]{000000} 14.92}                         & {\color[HTML]{000000} 0.6873}                         & {\color[HTML]{000000} 0.3950}                         & {\color[HTML]{000000} 13.84}                         & {\color[HTML]{000000} 0.6556}                         & {\color[HTML]{000000} 0.4170}                         \\
                                                                           &                          & GO-Surf                   & {\color[HTML]{000000} 0.0306}                         & {\color[HTML]{000000} 0.0369}                         & {\color[HTML]{000000} 0.0337}                         & {\color[HTML]{000000} 0.8659}                         & {\color[HTML]{000000} 0.8099}                         & {\color[HTML]{000000} 21.48}                         & {\color[HTML]{000000} 0.7698}                         & {\color[HTML]{000000} 0.2685}                         & {\color[HTML]{000000} 19.45}                         & {\color[HTML]{000000} 0.7189}                         & {\color[HTML]{000000} 0.2332}                         \\
                                                                           &                          & Nerfacto                  & {\color[HTML]{000000} 0.0349}                         & {\color[HTML]{000000} 0.2015}                         & {\color[HTML]{000000} 0.1182}                         & {\color[HTML]{000000} 0.7018}                         & {\color[HTML]{000000} 0.5870}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 22.99} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.7918} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.2245} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 22.95} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.8564} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.1276} \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0136} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0161} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0149} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.9130} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.9655} & {\color[HTML]{000000} 21.21}                         & {\color[HTML]{000000} 0.7709}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.2132} & {\color[HTML]{000000} 21.98}                         & {\color[HTML]{000000} 0.8465}                         & {\color[HTML]{000000} 0.1427}                         \\
                                                                           & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0139} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0167} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0153} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.9108} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.9625} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 22.95} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.7946} & {\color[HTML]{000000} 0.2396}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 22.99} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.8579} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.1354} \\ \cline{2-14} 
                                                                           &                          & Volumetric Fusion         & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.0355} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.0187} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.0271} & {\color[HTML]{330001} 0.7990}                         & {\color[HTML]{330001} 0.8616}                         & {\color[HTML]{330001} 12.01}                         & {\color[HTML]{330001} 0.5546}                         & {\color[HTML]{330001} 0.4869}                         & {\color[HTML]{330001} 12.35}                         & {\color[HTML]{330001} 0.5849}                         & {\color[HTML]{330001} 0.4695}                         \\
                                                                           &                          & GO-Surf                   & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.0278} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.0229} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.0254} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.8767} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.9248} & {\color[HTML]{330001} 18.88}                         & {\color[HTML]{330001} 0.6726}                         & {\color[HTML]{330001} 0.3659}                         & {\color[HTML]{330001} 18.42}                         & {\color[HTML]{330001} 0.6764}                         & {\color[HTML]{330001} 0.3940}                         \\
                                                                           &                          & Nerfacto                  & {\color[HTML]{330001} 0.0406}                         & {\color[HTML]{330001} 0.3443}                         & {\color[HTML]{330001} 0.1924}                         & {\color[HTML]{330001} 0.6573}                         & {\color[HTML]{330001} 0.4773}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 21.22} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.7884} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.2040} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 22.35} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.8136} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{330001} 0.2159} \\
                                                                           &                          & NeuS-facto                & {\color[HTML]{330001} 0.0407}                         & {\color[HTML]{330001} 0.0231}                         & {\color[HTML]{330001} 0.0319}                         & {\color[HTML]{330001} 0.8604}                         & {\color[HTML]{330001} 0.8884}                         & {\color[HTML]{330001} 19.44}                         & {\color[HTML]{330001} 0.7250}                         & {\color[HTML]{330001} 0.3463}                         & {\color[HTML]{330001} 20.01}                         & {\color[HTML]{330001} 0.7230}                         & {\color[HTML]{330001} 0.3631}                         \\
\multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}coffee\\ room\end{tabular}}   & \multirow{-5}{*}{iPhone} & Ous                       & {\color[HTML]{330001} 0.0412}                         & {\color[HTML]{330001} 0.0234}                         & {\color[HTML]{330001} 0.0323}                         & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.8653} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.8892} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 20.89} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.7564} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.2968} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 21.38} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.7636} & \cellcolor[HTML]{FFD966}{\color[HTML]{330001} 0.2961} \\ \hline
                                                                           &                          & Volumetric Fusion         & {\color[HTML]{000000} 0.0323}                         & {\color[HTML]{000000} 0.0402}                         & {\color[HTML]{000000} 0.0362}                         & {\color[HTML]{000000} 0.8402}                         & {\color[HTML]{000000} 0.8395}                         & {\color[HTML]{000000} 15.41}                         & {\color[HTML]{000000} 0.6764}                         & {\color[HTML]{000000} 0.4007}                         & {\color[HTML]{000000} 14.87}                         & {\color[HTML]{000000} 0.6867}                         & {\color[HTML]{000000} 0.4086}                         \\
                                                                           &                          & GO-Surf                   & {\color[HTML]{000000} 0.0281}                         & {\color[HTML]{000000} 0.0302}                         & {\color[HTML]{000000} 0.0291}                         & {\color[HTML]{000000} 0.9016}                         & {\color[HTML]{000000} 0.8972}                         & {\color[HTML]{000000} 22.40}                         & {\color[HTML]{000000} 0.7877}                         & {\color[HTML]{000000} 0.2615}                         & {\color[HTML]{000000} 22.44}                         & {\color[HTML]{000000} 0.8178}                         & {\color[HTML]{000000} 0.2305}                         \\
                                                                           &                          & Nerfacto                  & {\color[HTML]{000000} 0.0556}                         & {\color[HTML]{000000} 0.1008}                         & {\color[HTML]{000000} 0.0782}                         & {\color[HTML]{000000} 0.7314}                         & {\color[HTML]{000000} 0.5985}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 24.15} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.8270} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.2094} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 26.29} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.8849} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.1510} \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0253} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0229} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0241} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.9033} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.9122} & {\color[HTML]{000000} 22.99}                         & {\color[HTML]{000000} 0.8080}                         & {\color[HTML]{000000} 0.2338}                         & {\color[HTML]{000000} 25.00}                         & {\color[HTML]{000000} 0.8561}                         & {\color[HTML]{000000} 0.1925}                         \\
                                                                           & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0258} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0233} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0246} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.9018} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.9106} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 24.05} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.8262} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.2285} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 25.65} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.8722} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.1787} \\ \cline{2-14} 
                                                                           &                          & Volumetric Fusion         & {\color[HTML]{000000} 0.0560}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0162} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0361} & {\color[HTML]{000000} 0.8069}                         & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.7925} & {\color[HTML]{000000} 12.29}                         & {\color[HTML]{000000} 0.6000}                         & {\color[HTML]{000000} 0.4543}                         & {\color[HTML]{000000} 11.96}                         & {\color[HTML]{000000} 0.5596}                         & {\color[HTML]{000000} 0.4635}                         \\
                                                                           &                          & GO-Surf                   & {\color[HTML]{000000} 0.0646}                         & {\color[HTML]{000000} 0.0407}                         & {\color[HTML]{000000} 0.0526}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.8566} & {\color[HTML]{000000} 0.6302}                         & {\color[HTML]{000000} 17.90}                         & {\color[HTML]{000000} 0.6768}                         & {\color[HTML]{000000} 0.3847}                         & {\color[HTML]{000000} 16.59}                         & {\color[HTML]{000000} 0.5820}                         & {\color[HTML]{000000} 0.4886}                         \\
                                                                           &                          & Nerfacto                  & {\color[HTML]{000000} 0.0623}                         & {\color[HTML]{000000} 0.1471}                         & {\color[HTML]{000000} 0.1047}                         & {\color[HTML]{000000} 0.6432}                         & {\color[HTML]{000000} 0.5684}                         & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 21.94} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.7855} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.2393} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 21.86} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.7903} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.2159} \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0551} & {\color[HTML]{000000} 0.0299}                         & {\color[HTML]{000000} 0.0425}                         & {\color[HTML]{000000} 0.8452}                         & {\color[HTML]{000000} 0.7854}                         & {\color[HTML]{000000} 16.59}                         & {\color[HTML]{000000} 0.6636}                         & {\color[HTML]{000000} 0.4197}                         & {\color[HTML]{000000} 15.83}                         & {\color[HTML]{000000} 0.6327}                         & {\color[HTML]{000000} 0.4321}                         \\
\multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}computer\\ room\end{tabular}} & \multirow{-5}{*}{iPhone} & Ous                       & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.0474} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0276} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.0375} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.8555} & \cellcolor[HTML]{FFC7CE}{\color[HTML]{000000} 0.8172} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 20.10} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.7411} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.3530} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 18.10} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.6894} & \cellcolor[HTML]{FFD966}{\color[HTML]{000000} 0.3649} \\ \hline
                                                                           &                          & Volumetric Fusion         & 0.0469                                                & 0.0431                                                & 0.0450                                                & 0.7633                                                & 0.7658                                                & 12.46                                                & 0.5750                                                & 0.4898                                                & 12.09                                                & 0.5455                                                & 0.5273                                                \\
                                                                           &                          & GO-Surf                   & 0.0401                                                & \cellcolor[HTML]{FFC7CE}0.0258                        & \cellcolor[HTML]{FFC7CE}0.0330                        & 0.8118                                                & \cellcolor[HTML]{FFC7CE}0.8816                        & 18.99                                                & 0.6985                                                & 0.3823                                                & 19.42                                                & 0.7283                                                & 0.3120                                                \\
                                                                           &                          & Nerfacto                  & 0.0564                                                & 0.1043                                                & 0.0804                                                & 0.7089                                                & 0.6258                                                & \cellcolor[HTML]{FFC7CE}21.12                        & \cellcolor[HTML]{FFC7CE}0.7535                        & \cellcolor[HTML]{FFC7CE}0.2908                        & \cellcolor[HTML]{FFC7CE}22.13                        & \cellcolor[HTML]{FFC7CE}0.8112                        & \cellcolor[HTML]{FFC7CE}0.2184                        \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}0.0384                        & \cellcolor[HTML]{FFD966}0.0320                        & \cellcolor[HTML]{FFD966}0.0352                        & \cellcolor[HTML]{FFD966}0.8150                        & \cellcolor[HTML]{FFD966}0.8468                        & 19.53                                                & 0.7258                                                & 0.3356                                                & 20.18                                                & 0.7707                                                & 0.2750                                                \\
                                                                           & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFC7CE}0.0377                        & 0.0332                                                & 0.0354                                                & \cellcolor[HTML]{FFC7CE}0.8151                        & 0.8455                                                & \cellcolor[HTML]{FFD966}20.89                        & \cellcolor[HTML]{FFD966}0.7509                        & \cellcolor[HTML]{FFD966}0.3221                        & \cellcolor[HTML]{FFD966}21.33                        & \cellcolor[HTML]{FFD966}0.7919                        & \cellcolor[HTML]{FFD966}0.2534                        \\ \cline{2-14} 
                                                                           &                          & Volumetric Fusion         & \cellcolor[HTML]{FFC7CE}0.0688                        & \cellcolor[HTML]{FFC7CE}0.0238                        & \cellcolor[HTML]{FFC7CE}0.0463                        & 0.7344                                                & \cellcolor[HTML]{FFC7CE}0.7479                        & 11.27                                                & 0.4335                                                & 0.5815                                                & 11.08                                                & 0.4542                                                & 0.5731                                                \\
                                                                           &                          & GO-Surf                   & 0.1045                                                & \cellcolor[HTML]{FFD966}0.0347                        & 0.0696                                                & \cellcolor[HTML]{FFC7CE}0.7592                        & \cellcolor[HTML]{FFD966}0.6494                        & 15.36                                                & 0.4892                                                & 0.5902                                                & 14.31                                                & 0.4928                                                & 0.6094                                                \\
                                                                           &                          & Nerfacto                  & \cellcolor[HTML]{FFD966}0.0709                        & 0.1334                                                & 0.1022                                                & 0.6608                                                & 0.6430                                                & \cellcolor[HTML]{FFC7CE}18.27                        & \cellcolor[HTML]{FFC7CE}0.6381                        & \cellcolor[HTML]{FFC7CE}0.3617                        & \cellcolor[HTML]{FFC7CE}17.05                        & \cellcolor[HTML]{FFC7CE}0.6003                        & \cellcolor[HTML]{FFC7CE}0.4137                        \\
                                                                           &                          & NeuS-facto                & 0.0938                                                & 0.0585                                                & 0.0761                                                & 0.7290                                                & 0.5719                                                & 15.61                                                & 0.5391                                                & 0.5654                                                & 14.23                                                & 0.5153                                                & 0.5743                                                \\
\multirow{-10}{*}{activity}                                                & \multirow{-5}{*}{iPhone} & Ous                       & 0.0837                                                & 0.0536                                                & \cellcolor[HTML]{FFD966}0.0687                        & \cellcolor[HTML]{FFD966}0.7505                        & 0.6108                                                & \cellcolor[HTML]{FFD966}16.64                        & \cellcolor[HTML]{FFD966}0.5748                        & \cellcolor[HTML]{FFD966}0.5026                        & \cellcolor[HTML]{FFD966}15.30                        & \cellcolor[HTML]{FFD966}0.5641                        & \cellcolor[HTML]{FFD966}0.5274                        \\ \hline
                                                                           &                          & Volumetric Fusion         & 0.0426                                                & 0.0304                                                & 0.0365                                                & 0.7605                                                & 0.8316                                                & 14.51                                                & 0.6978                                                & 0.4051                                                & 12.36                                                & 0.6715                                                & 0.4362                                                \\
                                                                           &                          & GO-Surf                   & 0.0336                                                & 0.0311                                                & 0.0324                                                & \cellcolor[HTML]{FFC7CE}0.8173                        & 0.8823                                                & 20.61                                                & 0.8096                                                & 0.2907                                                & 18.21                                                & 0.7975                                                & 0.2881                                                \\
                                                                           &                          & Nerfacto                  & 0.0567                                                & 0.1361                                                & 0.0964                                                & 0.6144                                                & 0.5255                                                & \cellcolor[HTML]{FFD966}22.24                        & \cellcolor[HTML]{FFD966}0.8173                        & \cellcolor[HTML]{FFC7CE}0.2479                        & \cellcolor[HTML]{FFD966}20.34                        & \cellcolor[HTML]{FFD966}0.8554                        & \cellcolor[HTML]{FFC7CE}0.1972                        \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}0.0265                        & \cellcolor[HTML]{FFC7CE}0.0204                        & \cellcolor[HTML]{FFC7CE}0.0235                        & \cellcolor[HTML]{FFD966}0.8164                        & \cellcolor[HTML]{FFC7CE}0.9300                        & 20.94                                                & 0.8154                                                & 0.2654                                                & 19.18                                                & 0.8467                                                & 0.2138                                                \\
                                                                           & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}0.0272                        & \cellcolor[HTML]{FFD966}0.0209                        & \cellcolor[HTML]{FFD966}0.0240                        & 0.8142                                                & \cellcolor[HTML]{FFD966}0.9249                        & \cellcolor[HTML]{FFC7CE}22.25                        & \cellcolor[HTML]{FFC7CE}0.8226                        & \cellcolor[HTML]{FFD966}0.2619                        & \cellcolor[HTML]{FFC7CE}20.47                        & \cellcolor[HTML]{FFC7CE}0.8614                        & \cellcolor[HTML]{FFD966}0.2086                        \\ \cline{2-14} 
                                                                           &                          & Volumetric Fusion         & 0.0417                                                & \cellcolor[HTML]{FFC7CE}0.0149                        & \cellcolor[HTML]{FFC7CE}0.0283                        & 0.7688                                                & 0.8688                                                & 11.71                                                & 0.5719                                                & 0.5117                                                & 11.85                                                & 0.5564                                                & 0.5111                                                \\
                                                                           &                          & GO-Surf                   & 0.0513                                                & 0.0248                                                & 0.0381                                                & \cellcolor[HTML]{FFC7CE}0.8145                        & \cellcolor[HTML]{FFC7CE}0.8863                        & 17.11                                                & 0.6641                                                & 0.4564                                                & \cellcolor[HTML]{FFD966}18.58                        & 0.6730                                                & 0.4440                                                \\
                                                                           &                          & Nerfacto                  & 0.0554                                                & 0.0769                                                & 0.0661                                                & 0.6156                                                & 0.6376                                                & \cellcolor[HTML]{FFC7CE}18.14                        & \cellcolor[HTML]{FFC7CE}0.7492                        & \cellcolor[HTML]{FFC7CE}0.2939                        & \cellcolor[HTML]{FFC7CE}19.67                        & \cellcolor[HTML]{FFC7CE}0.7839                        & \cellcolor[HTML]{FFC7CE}0.2490                        \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}0.0394                        & \cellcolor[HTML]{FFD966}0.0219                        & \cellcolor[HTML]{FFD966}0.0307                        & 0.7946                                                & \cellcolor[HTML]{FFD966}0.8746                        & 15.64                                                & 0.6806                                                & 0.4440                                                & 16.45                                                & 0.6624                                                & 0.4312                                                \\
\multirow{-10}{*}{kokko}                                                   & \multirow{-5}{*}{iPhone} & Ous                       & \cellcolor[HTML]{FFD966}0.0398                        & 0.0248                                                & 0.0323                                                & \cellcolor[HTML]{FFD966}0.8019                        & 0.8651                                                & \cellcolor[HTML]{FFD966}17.65                        & \cellcolor[HTML]{FFD966}0.7280                        & \cellcolor[HTML]{FFD966}0.3865                        & 17.72                                                & \cellcolor[HTML]{FFD966}0.6814                        & \cellcolor[HTML]{FFD966}0.3711                        \\ \hline
                                                                           &                          & Volumetric Fusion         & 0.0265                                                & 0.0307                                                & 0.0286                                                & 0.8404                                                & 0.8759                                                & 13.30                                                & 0.6668                                                & 0.4357                                                & 12.20                                                & 0.6902                                                & 0.4233                                                \\
                                                                           &                          & GO-Surf                   & 0.0230                                                & \cellcolor[HTML]{FFD966}0.0189                        & 0.0209                                                & \cellcolor[HTML]{FFD966}0.9006                        & \cellcolor[HTML]{FFD966}0.9401                        & 19.43                                                & 0.7871                                                & 0.2946                                                & 20.99                                                & 0.7976                                                & 0.2449                                                \\
                                                                           &                          & Nerfacto                  & 0.0476                                                & 0.1599                                                & 0.1038                                                & 0.6742                                                & 0.6076                                                & \cellcolor[HTML]{FFC7CE}21.00                        & \cellcolor[HTML]{FFD966}0.7949                        & \cellcolor[HTML]{FFC7CE}0.2374                        & \cellcolor[HTML]{FFD966}22.88                        & \cellcolor[HTML]{FFD966}0.8619                        & \cellcolor[HTML]{FFD966}0.1533                        \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}0.0185                        & \cellcolor[HTML]{FFC7CE}0.0184                        & \cellcolor[HTML]{FFC7CE}0.0184                        & \cellcolor[HTML]{FFC7CE}0.9024                        & \cellcolor[HTML]{FFC7CE}0.9403                        & 19.40                                                & 0.7759                                                & 0.2658                                                & 22.45                                                & 0.8505                                                & 0.1616                                                \\
                                                                           & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}0.0191                        & \cellcolor[HTML]{FFD966}0.0189                        & \cellcolor[HTML]{FFD966}0.0190                        & 0.9002                                                & 0.9354                                                & \cellcolor[HTML]{FFD966}20.86                        & \cellcolor[HTML]{FFC7CE}0.8000                        & \cellcolor[HTML]{FFD966}0.2584                        & \cellcolor[HTML]{FFC7CE}23.59                        & \cellcolor[HTML]{FFC7CE}0.8683                        & \cellcolor[HTML]{FFC7CE}0.1527                        \\ \cline{2-14} 
                                                                           &                          & Volumetric Fusion         & 0.0378                                                & \cellcolor[HTML]{FFC7CE}0.0134                        & \cellcolor[HTML]{FFC7CE}0.0256                        & 0.8184                                                & 0.8712                                                & 11.47                                                & 0.5243                                                & 0.5268                                                & 11.88                                                & 0.5479                                                & 0.5183                                                \\
                                                                           &                          & GO-Surf                   & 0.0414                                                & 0.0332                                                & 0.0373                                                & 0.8729                                                & 0.8627                                                & 17.35                                                & 0.6037                                                & 0.4502                                                & 17.10                                                & 0.6267                                                & 0.4529                                                \\
                                                                           &                          & Nerfacto                  & \cellcolor[HTML]{FFC7CE}0.0266                        & 0.2674                                                & 0.1470                                                & 0.6725                                                & 0.6064                                                & \cellcolor[HTML]{FFC7CE}19.34                        & \cellcolor[HTML]{FFC7CE}0.7414                        & \cellcolor[HTML]{FFC7CE}0.2391                        & \cellcolor[HTML]{FFC7CE}19.46                        & \cellcolor[HTML]{FFC7CE}0.7605                        & \cellcolor[HTML]{FFC7CE}0.2203                        \\
                                                                           &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}0.0316                        & \cellcolor[HTML]{FFD966}0.0195                        & \cellcolor[HTML]{FFC7CE}0.0256                        & \cellcolor[HTML]{FFD966}0.8803                        & \cellcolor[HTML]{FFC7CE}0.9093                        & 17.35                                                & 0.6671                                                & 0.3593                                                & 18.02                                                & 0.6810                                                & 0.3448                                                \\
\multirow{-10}{*}{honka}                                                   & \multirow{-5}{*}{iPhone} & Ous                       & 0.0329                                                & 0.0258                                                & 0.0294                                                & \cellcolor[HTML]{FFC7CE}0.8820                        & \cellcolor[HTML]{FFD966}0.8887                        & \cellcolor[HTML]{FFD966}18.89                        & \cellcolor[HTML]{FFD966}0.7054                        & \cellcolor[HTML]{FFD966}0.3136                        & \cellcolor[HTML]{FFD966}18.25                        & \cellcolor[HTML]{FFD966}0.6978                        & \cellcolor[HTML]{FFD966}0.3155                        \\ \hline
\end{tabular}%
}
\caption{The quantitative reconstruction and rendering comparison results of each room. The best results are highlighted in pink. The second best results are marked in yellow. Test within a single sequence means we uniformly sample test frames from a single sequence and train on all left frames. Test with a different sequence means we train on one sequence and test on another individual sequence. Our method provides a good trade-off between mesh and novel view synthesis results.}
\label{cmp1}
\end{table*}

==> WACVAuthorKit/sec/exp/comparison2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table.xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option. i.e. \documentclass[xcolor=table]{beamer}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table.xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table.xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccc}
\hline
                             &                          &                           & \multicolumn{5}{c}{}                                                                                                                                               & \multicolumn{6}{c}{Rendering quality}                                                                                                                                                             \\ \cline{9-14} 
                             &                          &                           & \multicolumn{5}{c}{\multirow{-2}{*}{Reconstruction quality}}                                                                                                       & \multicolumn{3}{c}{Test within a single sequence}                                               & \multicolumn{3}{c}{Test with a different sequence}                                              \\ \cline{4-14} 
\multirow{-3}{*}{Room}       & \multirow{-3}{*}{Device} & \multirow{-3}{*}{Methods} & \textbf{Acc} $\downarrow$                           & \textbf{Comp} $\downarrow$                          & \textbf{C-}$\ell_1$ $\downarrow$                          & \textbf{NC} $\uparrow$                            & \textbf{F-score} $\uparrow$                      & \textbf{PSNR} $\uparrow$                         & \textbf{SSIM} $\uparrow$                         & \textbf{LPIPS} $\downarrow$                        & \textbf{PSNR} $\uparrow$                         & \textbf{SSIM} $\uparrow$                         & \textbf{LPIPS} $\downarrow$                        \\ \hline
                             &                          & Volumetric Fusion         & 0.0365                         & 0.0288                         & 0.0327                         & 0.8233                         & 0.8398                         & 14.56                         & 0.7024                         & 0.3721                         & 13.54                         & 0.6751                         & 0.4106                         \\
                             &                          & GO-Surf                   & 0.0310                         & \cellcolor[HTML]{FFC7CE}0.0221 & 0.0265                         & \cellcolor[HTML]{FFC7CE}0.8836 & \cellcolor[HTML]{FFC7CE}0.8998 & 22.85                         & 0.8109                         & 0.2419                         & 22.22                         & 0.7921                         & 0.2017                         \\
                             &                          & Nerfacto                  & 0.0567                         & 0.1697                         & 0.1132                         & 0.6968                         & 0.5461                         & \cellcolor[HTML]{FFC7CE}24.96 & \cellcolor[HTML]{FFC7CE}0.8420 & \cellcolor[HTML]{FFC7CE}0.1989 & \cellcolor[HTML]{FFC7CE}25.80 & \cellcolor[HTML]{FFC7CE}0.8920 & \cellcolor[HTML]{FFC7CE}0.1277 \\
                             &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}0.0296 & \cellcolor[HTML]{FFC7CE}0.0221 & \cellcolor[HTML]{FFC7CE}0.0259 & 0.8785                         & \cellcolor[HTML]{FFD966}0.8879 & 23.10                         & 0.8238                         & 0.2458                         & 24.16                         & 0.8696                         & 0.1552                         \\
                             & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}0.0298 & 0.0223                         & \cellcolor[HTML]{FFD966}0.0260 & \cellcolor[HTML]{FFD966}0.8789 & 0.8853                         & \cellcolor[HTML]{FFD966}24.66 & \cellcolor[HTML]{FFD966}0.8401 & \cellcolor[HTML]{FFD966}0.2270 & \cellcolor[HTML]{FFD966}25.44 & \cellcolor[HTML]{FFD966}0.8812 & \cellcolor[HTML]{FFD966}0.1471 \\ \cline{2-14} 
                             &                          & Volumetric Fusion         & 0.0592                         & \cellcolor[HTML]{FFC7CE}0.0209 & \cellcolor[HTML]{FFC7CE}0.0401 & 0.7736                         & \cellcolor[HTML]{FFD966}0.7457 & 11.32                         & 0.5425                         & 0.5362                         & 11.43                         & 0.5337                         & 0.5219                         \\
                             &                          & GO-Surf                   & \cellcolor[HTML]{FFC7CE}0.0511 & \cellcolor[HTML]{FFD966}0.0308 & \cellcolor[HTML]{FFD966}0.0410 & \cellcolor[HTML]{FFC7CE}0.8563 & \cellcolor[HTML]{FFC7CE}0.7725 & 17.40                         & 0.6042                         & 0.5191                         & \cellcolor[HTML]{FFD966}19.27 & 0.6482                         & 0.4793                         \\
                             &                          & Nerfacto                  & \cellcolor[HTML]{FFD966}0.0519 & 0.1311                         & 0.0915                         & 0.6976                         & 0.6339                         & \cellcolor[HTML]{FFC7CE}20.63 & \cellcolor[HTML]{FFC7CE}0.7095 & \cellcolor[HTML]{FFC7CE}0.3463 & \cellcolor[HTML]{FFC7CE}22.54 & \cellcolor[HTML]{FFC7CE}0.7900 & \cellcolor[HTML]{FFC7CE}0.2339 \\
                             &                          & NeuS-facto                & 0.0596                         & 0.0446                         & 0.0521                         & 0.8047                         & 0.6781                         & 17.72                         & 0.6559                         & 0.5018                         & 18.52                         & \cellcolor[HTML]{FFD966}0.6833 & 0.4602                         \\
\multirow{-10}{*}{classroom} & \multirow{-5}{*}{iPhone} & Ours                      & 0.0546                         & 0.0402                         & 0.0474                         & \cellcolor[HTML]{FFD966}0.8130 & 0.7088                         & \cellcolor[HTML]{FFD966}19.63 & \cellcolor[HTML]{FFD966}0.6901 & \cellcolor[HTML]{FFD966}0.4464 & 19.23                         & 0.6729                         & \cellcolor[HTML]{FFD966}0.3824 \\ \hline
                             &                          & Volumetric Fusion         & \cellcolor[HTML]{FFC7CE}0.0664 & 0.0344                         & 0.0504                         & 0.7953                         & 0.7979                         & 12.97                         & 0.6039                         & 0.4701                         & 11.94                         & 0.6087                         & 0.4795                         \\
                             &                          & GO-Surf                   & 0.0815                         & 0.0398                         & 0.0606                         & 0.8501                         & 0.8046                         & 20.31                         & 0.7393                         & 0.2873                         & 19.31                         & 0.7273                         & 0.3268                         \\
                             &                          & Nerfacto                  & 0.0927                         & 0.0924                         & 0.0925                         & 0.6793                         & 0.5664                         & \cellcolor[HTML]{FFD966}21.49 & \cellcolor[HTML]{FFD966}0.7696 & \cellcolor[HTML]{FFC7CE}0.2466 & \cellcolor[HTML]{FFD966}20.18 & \cellcolor[HTML]{FFC7CE}0.7571 & \cellcolor[HTML]{FFC7CE}0.2663 \\
                             &                          & NeuS-facto                & 0.0749                         & \cellcolor[HTML]{FFD966}0.0231 & \cellcolor[HTML]{FFD966}0.0490 & \cellcolor[HTML]{FFD966}0.8506 & \cellcolor[HTML]{FFD966}0.8485 & 19.99                         & 0.7460                         & \cellcolor[HTML]{FFD966}0.2590 & 19.51                         & 0.7397                         & \cellcolor[HTML]{FFD966}0.2732 \\
                             & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFD966}0.0737 & \cellcolor[HTML]{FFC7CE}0.0228 & \cellcolor[HTML]{FFC7CE}0.0482 & \cellcolor[HTML]{FFC7CE}0.8507 & \cellcolor[HTML]{FFC7CE}0.8491 & \cellcolor[HTML]{FFC7CE}21.63 & \cellcolor[HTML]{FFC7CE}0.7707 & 0.2649                         & \cellcolor[HTML]{FFC7CE}20.19 & \cellcolor[HTML]{FFD966}0.7553 & 0.2841                         \\ \cline{2-14} 
                             &                          & Volumetric Fusion         & \cellcolor[HTML]{FFC7CE}0.0843 & \cellcolor[HTML]{FFC7CE}0.0286 & \cellcolor[HTML]{FFC7CE}0.0564 & 0.7629                         & \cellcolor[HTML]{FFD966}0.7108 & 11.82                         & 0.5597                         & 0.4896                         & 11.89                         & 0.5335                         & 0.5313                         \\
                             &                          & GO-Surf                   & \cellcolor[HTML]{FFD966}0.0906 & \cellcolor[HTML]{FFD966}0.0320 & \cellcolor[HTML]{FFD966}0.0613 & \cellcolor[HTML]{FFC7CE}0.8106 & \cellcolor[HTML]{FFC7CE}0.7116 & 16.42                         & 0.6263                         & 0.4140                         & 15.50                         & 0.5589                         & 0.5198                         \\
                             &                          & Nerfacto                  & 0.1004                         & 0.1053                         & 0.1028                         & 0.6452                         & 0.5358                         & \cellcolor[HTML]{FFC7CE}20.68 & \cellcolor[HTML]{FFC7CE}0.7862 & \cellcolor[HTML]{FFC7CE}0.2150 & \cellcolor[HTML]{FFC7CE}19.07 & \cellcolor[HTML]{FFC7CE}0.7057 & \cellcolor[HTML]{FFC7CE}0.3112 \\
                             &                          & NeuS-facto                & 0.1021                         & 0.0417                         & 0.0719                         & 0.7808                         & 0.6454                         & 17.13                         & 0.6983                         & 0.3764                         & 16.04                         & 0.6365                         & 0.4552                         \\
\multirow{-10}{*}{koivu}     & \multirow{-5}{*}{iPhone} & Ours                      & 0.0924                         & 0.0418                         & 0.0671                         & \cellcolor[HTML]{FFD966}0.7984 & 0.6758                         & \cellcolor[HTML]{FFD966}19.94 & \cellcolor[HTML]{FFD966}0.7491 & \cellcolor[HTML]{FFD966}0.3059 & \cellcolor[HTML]{FFD966}18.04 & \cellcolor[HTML]{FFD966}0.6753 & \cellcolor[HTML]{FFD966}0.3938 \\ \hline
                             &                          & Volumetric Fusion         & 0.0199                         & 0.0206                         & 0.0202                         & 0.8580                         & 0.9003                         & 14.32                         & 0.7514                         & 0.3708                         & 14.37                         & 0.7632                         & 0.3785                         \\
                             &                          & GO-Surf                   & 0.0291                         & 0.0808                         & 0.0550                         & 0.8706                         & 0.7273                         & 22.56                         & 0.8429                         & 0.2750                         & 20.05                         & 0.8112                         & 0.3058                         \\
                             &                          & Nerfacto                  & 0.0501                         & 0.2916                         & 0.1709                         & 0.6608                         & 0.4312                         & \cellcolor[HTML]{FFD966}24.25 & \cellcolor[HTML]{FFD966}0.8565 & \cellcolor[HTML]{FFD966}0.2038 & \cellcolor[HTML]{FFC7CE}24.90 & \cellcolor[HTML]{FFC7CE}0.9009 & \cellcolor[HTML]{FFC7CE}0.1384 \\
                             &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}0.0152 & \cellcolor[HTML]{FFD966}0.0186 & \cellcolor[HTML]{FFD966}0.0169 & 0.9126                         & \cellcolor[HTML]{FFD966}0.9376 & 22.65                         & 0.8502                         & 0.2351                         & 23.55                         & 0.8928                         & 0.1658                         \\
                             & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFC7CE}0.0151 & \cellcolor[HTML]{FFC7CE}0.0185 & \cellcolor[HTML]{FFC7CE}0.0168 & \cellcolor[HTML]{FFC7CE}0.9135 & \cellcolor[HTML]{FFC7CE}0.9378 & \cellcolor[HTML]{FFC7CE}26.46 & \cellcolor[HTML]{FFC7CE}0.9081 & \cellcolor[HTML]{FFC7CE}0.1546 & \cellcolor[HTML]{FFD966}24.69 & \cellcolor[HTML]{FFD966}0.8995 & \cellcolor[HTML]{FFD966}0.1589 \\ \cline{2-14} 
                             &                          & Volumetric Fusion         & 0.0381                         & \cellcolor[HTML]{FFC7CE}0.0158 & \cellcolor[HTML]{FFD966}0.0270 & 0.8177                         & 0.8347                         & 11.57                         & 0.5975                         & 0.5157                         & 11.44                         & 0.6022                         & 0.5151                         \\
                             &                          & GO-Surf                   & \cellcolor[HTML]{FFC7CE}0.0281 & 0.0222                         & \cellcolor[HTML]{FFC7CE}0.0252 & \cellcolor[HTML]{FFC7CE}0.8932 & \cellcolor[HTML]{FFC7CE}0.8795 & 19.64                         & 0.6920                         & 0.4356                         & \cellcolor[HTML]{FFD966}19.69 & 0.7133                         & 0.4240                         \\
                             &                          & Nerfacto                  & 0.0427                         & 0.0705                         & 0.0566                         & 0.7026                         & 0.6719                         & \cellcolor[HTML]{FFC7CE}22.62 & \cellcolor[HTML]{FFC7CE}0.8254 & \cellcolor[HTML]{FFC7CE}0.2244 & \cellcolor[HTML]{FFC7CE}22.17 & \cellcolor[HTML]{FFC7CE}0.8095 & \cellcolor[HTML]{FFC7CE}0.2570 \\
                             &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}0.0330 & \cellcolor[HTML]{FFD966}0.0219 & 0.0274                         & 0.8818                         & \cellcolor[HTML]{FFD966}0.8535 & 20.60                         & 0.7705                         & 0.3568                         & 18.63                         & 0.7055                         & 0.3965                         \\
\multirow{-10}{*}{vr room}   & \multirow{-5}{*}{iPhone} & Ours                      & 0.0336                         & 0.0226                         & 0.0281                         & \cellcolor[HTML]{FFD966}0.8831 & 0.8483                         & \cellcolor[HTML]{FFD966}22.04 & \cellcolor[HTML]{FFD966}0.7937 & \cellcolor[HTML]{FFD966}0.3088 & 19.45                         & \cellcolor[HTML]{FFD966}0.7178 & \cellcolor[HTML]{FFD966}0.3477 \\ \hline
                             &                          & Volumetric Fusion         & 0.0240                         & 0.0395                         & 0.0317                         & 0.8461                         & 0.8790                         & 13.60                         & 0.6623                         & 0.4127                         & 13.22                         & 0.6549                         & 0.4232                         \\
                             &                          & GO-Surf                   & 0.0233                         & 0.0394                         & 0.0314                         & 0.9003                         & 0.9124                         & 19.32                         & 0.7551                         & 0.3788                         & 18.35                         & 0.7622                         & 0.3539                         \\
                             &                          & Nerfacto                  & 0.0590                         & 0.1231                         & 0.0910                         & 0.6892                         & 0.6433                         & \cellcolor[HTML]{FFD966}19.81 & \cellcolor[HTML]{FFD966}0.7688 & \cellcolor[HTML]{FFD966}0.3329 & \cellcolor[HTML]{FFD966}19.07 & 0.7833                         & \cellcolor[HTML]{FFC7CE}0.2690 \\
                             &                          & NeuS-facto                & \cellcolor[HTML]{FFD966}0.0185 & \cellcolor[HTML]{FFD966}0.0349 & \cellcolor[HTML]{FFD966}0.0267 & \cellcolor[HTML]{FFD966}0.9010 & \cellcolor[HTML]{FFC7CE}0.9235 & 18.53                         & 0.7553                         & 0.3510                         & 18.69                         & \cellcolor[HTML]{FFD966}0.7884 & \cellcolor[HTML]{FFD966}0.2817 \\
                             & \multirow{-5}{*}{Kinect} & Ours                      & \cellcolor[HTML]{FFC7CE}0.0181 & \cellcolor[HTML]{FFC7CE}0.0348 & \cellcolor[HTML]{FFC7CE}0.0265 & \cellcolor[HTML]{FFC7CE}0.9052 & \cellcolor[HTML]{FFD966}0.9227 & \cellcolor[HTML]{FFC7CE}20.21 & \cellcolor[HTML]{FFC7CE}0.7750 & \cellcolor[HTML]{FFC7CE}0.3242 & \cellcolor[HTML]{FFC7CE}19.11 & \cellcolor[HTML]{FFC7CE}0.7896 & 0.2848                         \\ \cline{2-14} 
                             &                          & Volumetric Fusion         & \cellcolor[HTML]{FFC7CE}0.0387 & \cellcolor[HTML]{FFC7CE}0.0203 & \cellcolor[HTML]{FFC7CE}0.0295 & 0.8312                         & \cellcolor[HTML]{FFC7CE}0.8537 & 12.16                         & 0.5739                         & 0.5277                         & 11.99                         & 0.5874                         & 0.5135                         \\
                             &                          & GO-Surf                   & 0.0672                         & \cellcolor[HTML]{FFD966}0.0279 & \cellcolor[HTML]{FFD966}0.0476 & \cellcolor[HTML]{FFC7CE}0.8699 & \cellcolor[HTML]{FFD966}0.8206 & 18.93                         & 0.6581                         & 0.4927                         & \cellcolor[HTML]{FFD966}18.76 & 0.6736                         & 0.4967                         \\
                             &                          & Nerfacto                  & \cellcolor[HTML]{FFD966}0.0609 & 0.0933                         & 0.0771                         & 0.6696                         & 0.6440                         & \cellcolor[HTML]{FFC7CE}21.19 & \cellcolor[HTML]{FFC7CE}0.7602 & \cellcolor[HTML]{FFC7CE}0.3131 & \cellcolor[HTML]{FFC7CE}21.43 & \cellcolor[HTML]{FFC7CE}0.7762 & \cellcolor[HTML]{FFC7CE}0.3156 \\
                             &                          & NeuS-facto                & 0.0630                         & 0.0436                         & 0.0533                         & 0.8357                         & 0.7241                         & 17.37                         & 0.6791                         & 0.5354                         & 16.78                         & 0.6585                         & 0.5330                         \\
\multirow{-10}{*}{sauna}     & \multirow{-5}{*}{iPhone} & Ours                      & 0.0648                         & 0.0509                         & 0.0579                         & \cellcolor[HTML]{FFD966}0.8480 & 0.6784                         & \cellcolor[HTML]{FFD966}19.82 & \cellcolor[HTML]{FFD966}0.7126 & \cellcolor[HTML]{FFD966}0.4700 & 18.61                         & \cellcolor[HTML]{FFD966}0.6805 & \cellcolor[HTML]{FFD966}0.4778 \\ \hline
                             &                          & Volumetric Fusion         & 0.0381                         & 0.0521                         & 0.0451                         & 0.7911                         & 0.7949                         & 12.34                         & 0.6049                         & 0.4563                         & 12.61                         & 0.5572                         & 0.5191                         \\
                             &                          & GO-Surf                   & \cellcolor[HTML]{FFD966}0.0345 & \cellcolor[HTML]{FFC7CE}0.0419 & \cellcolor[HTML]{FFC7CE}0.0382 & \cellcolor[HTML]{FFC7CE}0.8621 & \cellcolor[HTML]{FFC7CE}0.8648 & 17.63                         & 0.7074                         & 0.4143                         & 19.67                         & 0.7403                         & 0.3148                         \\
                             &                          & Nerfacto                  & 0.0599                         & 0.1056                         & 0.0827                         & 0.7216                         & 0.5836                         & \cellcolor[HTML]{FFC7CE}18.77 & \cellcolor[HTML]{FFD966}0.7497 & \cellcolor[HTML]{FFC7CE}0.2871 & \cellcolor[HTML]{FFC7CE}21.41 & \cellcolor[HTML]{FFC7CE}0.8538 & \cellcolor[HTML]{FFC7CE}0.1734 \\
                             &                          & NeuS-facto                & \cellcolor[HTML]{FFC7CE}0.0336 & \cellcolor[HTML]{FFD966}0.0446 & \cellcolor[HTML]{FFD966}0.0391 & 0.8453                         & \cellcolor[HTML]{FFD966}0.8324 & 17.77                         & 0.7281                         & 0.3550                         & 20.34                         & 0.8240                         & 0.2320                         \\
                             & \multirow{-5}{*}{Kinect} & Ours                      & 0.0346                         & 0.0466                         & 0.0406                         & \cellcolor[HTML]{FFD966}0.8454 & 0.8214                         & \cellcolor[HTML]{FFD966}18.62 & \cellcolor[HTML]{FFC7CE}0.7522 & \cellcolor[HTML]{FFD966}0.3271 & \cellcolor[HTML]{FFD966}21.05 & \cellcolor[HTML]{FFD966}0.8452 & \cellcolor[HTML]{FFD966}0.2078 \\ \cline{2-14} 
                             &                          & Volumetric Fusion         & \cellcolor[HTML]{FFC7CE}0.0610 & \cellcolor[HTML]{FFC7CE}0.0343 & \cellcolor[HTML]{FFC7CE}0.0477 & \cellcolor[HTML]{FFD966}0.7540 & \cellcolor[HTML]{FFC7CE}0.7632 & 11.78                         & 0.5613                         & \cellcolor[HTML]{FFD966}0.4957 & 12.12                         & 0.5656                         & \cellcolor[HTML]{FFD966}0.4771 \\
                             &                          & GO-Surf                   & 0.1033                         & \cellcolor[HTML]{FFD966}0.0361 & \cellcolor[HTML]{FFD966}0.0697 & \cellcolor[HTML]{FFC7CE}0.7914 & \cellcolor[HTML]{FFD966}0.6802 & 16.05                         & 0.6052                         & 0.5116                         & \cellcolor[HTML]{FFD966}18.21 & 0.6018                         & 0.5231                         \\
                             &                          & Nerfacto                  & \cellcolor[HTML]{FFD966}0.0798 & 0.0805                         & 0.0801                         & 0.6970                         & 0.5545                         & \cellcolor[HTML]{FFC7CE}21.31 & \cellcolor[HTML]{FFC7CE}0.7709 & \cellcolor[HTML]{FFC7CE}0.2589 & \cellcolor[HTML]{FFC7CE}21.63 & \cellcolor[HTML]{FFC7CE}0.7945 & \cellcolor[HTML]{FFC7CE}0.2377 \\
                             &                          & NeuS-facto                & 0.1405                         & 0.1484                         & 0.1445                         & 0.7228                         & 0.2688                         & 13.61                         & 0.6170                         & 0.5961                         & 13.80                         & 0.6058                         & 0.6174                         \\
\multirow{-10}{*}{olohuone}  & \multirow{-5}{*}{iPhone} & Ours                      & 0.1389                         & 0.1374                         & 0.1381                         & 0.7332                         & 0.2988                         & \cellcolor[HTML]{FFD966}17.27 & \cellcolor[HTML]{FFD966}0.6787 & 0.5140                         & 16.78                         & \cellcolor[HTML]{FFD966}0.6759 & 0.5079                         \\ \hline
\end{tabular}%
}
\caption{The quantitative reconstruction and rendering comparison results of each room. The best results are highlighted in pink. The second best results are marked in yellow. Test within a single sequence means we uniformly sample test frames from a single sequence and train on all left frames. Test with a different sequence means we train on one sequence and test on another individual sequence. Our method provides a good trade-off between mesh and novel view synthesis results.}
\label{cmp2}
\end{table*}
